AstroTimer: Rethinking Non-Access Stratum Timers in LEO Constellations

Low-Earth Orbit (LEO) constellations expand 5G coverage to remote regions but differ fundamentally from terrestrial networks due to rapidly changing topologies, fluctuating delays, and constrained onboard resources. Existing 3GPP Non-Access Stratum (NAS) timers, inherited from terrestrial and geostationary (GEO) or medium Earth orbit (MEO) systems, fail to accommodate these dynamics, leading to signaling storms and inefficiency. This paper introduces AstroTimer, a lightweight, adaptive framework for sizing NAS timers based on LEO-specific parameters such as link variability, processing delays, and network-function placement. AstroTimer derives a closed-form timer model with low computational cost and optimizes both watchdog and backoff timers for the 5G registration procedure. Simulation results demonstrate that AstroTimer significantly reduces registration time, retry frequency, and user equipment (UE) energy consumption compared to 3GPP defaults, while preventing signaling overloads. The proposed approach provides an operator-ready foundation for reliable, efficient, and scalable non-terrestrial 5G/6G deployments.

==> Sections/background.tex <==
%! Author = arshiya
%! Date = 4/11/25
\section{Background}\label{sec:background}

    In this section, we provide a brief overview of the initial registration procedure in 5G and the timers involved in this process.
    This procedure is required to request other services from the network.

    \subsection{Registration Call Flow}\label{subsec:registration-call-flow}
        After power-on, the UE initiates the registration procedure by transmitting a NAS \emph{Registration Request} to
        the Access and Mobility Management Function (AMF) via the Radio Access Network (RAN).
        Upon dispatching this message, the UE starts the T3510 timer and enters a waiting state.
        If the UE includes a valid temporary identifier and the RAN can resolve it to a known AMF, the RAN forwards the NAS message to that AMF.
        Otherwise, the RAN selects an appropriate AMF for initial registration.

        If the selected AMF differs from the one that previously served the UE—\eg{}, due to registration in a new tracking area—the new AMF initiates UE context transfer from the old AMF\@.
        The AMF then performs the authentication procedure to verify that the UE is legitimate and authorized to access the network.

        Once authenticated, the AMF registers itself as the serving AMF using the \emph{Nudm\_UECM} service, requests subscription data,
        and subscribes to updates via the \emph{Nudm\_SDM} service.
        It also retrieves UE-specific policy information from the Policy Control Function (PCF).

        If all procedures complete successfully, the AMF sends a NAS \emph{Registration Accept} to the UE.
        The UE then responds with a NAS \emph{Registration Complete} message, finalizing the registration process.

    \subsection{Timers in Registration}\label{subsec:timers-in-registration}

        Timers define how long an entity (such as UE or NF) should wait for a response before retransmitting a request, aborting the process, or transitioning to a recovery state.
        By restricting waiting times and limiting retries, timers help identify failures and regulate the signaling load.

        Now we explain the main timers that are involved in the registration process:

        \textbf{T3510}: Timer T3510 is initiated by the UE immediately after sending a Registration Request to the AMF to monitor the wait time for a response.
        If the UE receives a Registration Accept or Reject message within this period, it stops T3510 and proceeds accordingly.
        However, if T3510 expires without a response, the UE considers the registration attempt unsuccessful, aborts the
        procedure, and may release the NAS signaling connection.
        
        \textbf{T3560}: The purpose of this timer is to ensure the UE responds (with an Authentication Response or Authentication Failure) within a defined period.
        If the AMF does not receive a valid response before T3560 expires, it may retransmit the Authentication Request or abort the procedure.
        This mechanism helps detect unresponsive or unreachable UE early, preventing indefinite waiting.

        \textbf{T3550}: This timer is initiated by the AMF upon sending a Registration Accept message to the UE, awaiting the
        Registration Complete message.
        If T3550 expires without receiving this confirmation, the AMF may consider the registration incomplete and take appropriate actions.

        \textbf{T3502}: Defines the minimum waiting time before the UE can reattempt registration after a failure.
        This mechanism helps prevent network signaling overhead due to frequent registration attempts.
%        The UE begins the registration after power-on by sending an NAS Registration Request to the AMF via RAN\@.
%        If temporary UE identities are included and the RAN can map these to a valid AMF, the RAN forwards the NAS message to that AMF\@.
%        Otherwise, the RAN selects an AMF\@.
%        If a new AMF is selected (e.g., because the UE registers in an area not served by the old AMF), the new AMF retrieves the UE context from the old AMF\@.
%        The AMF performs the Authentication procedure to ensure that the UE is legitimate and legally authorized to get service from the network\@.
%        The AMF registers as serving AMF for the UE, using the \emph{Nudm\_UECM service}.
%        The AMF also requests subscription data and subscribes to subscription data updates using the \emph{Nudm\_SDM service}.
%        Then, the AMF retrieves UE policies from PCF\@.
%
%        If the Registration procedure is successful so far, the AMF provides a NAS Registration Accept to the UE.
%        Upon receiving the registration, the UE sends a NAS registration complete to the AMF\@.
%    \begin{table}[h] \caption[caption]{Timers in 5G NR}\label{tab:timers}
%    \vspace{-0.3cm}
%    \begin{center}
%        \begin{tabular}{|c|c|c|c|c|} \hline
%        Timer & Standard & WB-N1/CE & NR (MEO/GEO)  \\ \hline
%        T3510 & 15s  &  85s & 27s \\ \hline
%        T3511 & 10s  &  ? s & ? s \\\hline
%        T3550 & 6s    & 18s & 11s \\ \hline
%        T3502 & 12 min  &  &  \\ \hline
%        T3512 & 54 min &  &  \\\hline
%        T3517 &   &    &  \\ \hline
%        \end{tabular}\caption*{\hl{NB-N1 temporarily removed}}
%    \end{center}
%    \end{table}
%    In NB-N1 mode, the timer value shall be calculated using an NAS timer value that is network-dependent.
%
%    In this section, we are going to introduce timers of 5GS mobility and session management that we optimized in this paper
%    both on UE and CN sides, according to~\cite{NASTimers5G}.
%
%    \textbf{T3510}: Timer T3510 is initiated by the UE immediately after sending a Registration Request to the AMF to monitor the wait time for a response.
%    If the UE receives a Registration Accept or Reject message within this period, it stops T3510 and proceeds accordingly.
%    However, if T3510 expires without a response, the UE considers the registration attempt unsuccessful, aborts the
%    procedure, and may release the NAS signaling connection.
%
%    \textbf{T3550}: This timer is initiated by the AMF upon sending a Registration Accept message to the UE, awaiting the
%    Registration Complete message.
%    If T3550 expires without receiving this confirmation, the AMF may consider the registration incomplete and take appropriate actions.
%
%    \textbf{T3502}: Defines the minimum waiting time before the UE can reattempt registration after a failure.
%    This mechanism helps prevent network signaling overhead due to frequent registration attempts.
%
%    \textbf{T3512}: This timer governs the periodic registration updates from the UE to the network.
%    Upon expiry, the UE initiates a registration update to maintain its presence in the network.
%    The behavior of T3512 can vary based on network configurations, such as support for strictly periodic registration timers like NTNs.
%
%    \textbf{T3517}: Started by the UE after sending a Service Request message, T3517 monitors the wait time for a Service Accept or
%    Reject response from the AMF\@.
%    If the timer expires without a response, the UE may retry the request or consider the service attempt failed, depending on the specific procedure and network policies.
%        \textbf{T3560}: T3560 starts by AMF after transmission of \emph{Authentication Request} to the UE\@.
%        If the AMF receives a response from the UE before time expires, it proceeds\@.
%        Otherwise, it can take appropriate action such as \emph{Authentication Request} retransmission.

==> Tables/evaluation_resluts.tex <==
%! Author = arshiya
%! Date = 7/20/25
\begin{table}
    \caption{Evaluation Results}\label{tab:evaluation_results}
    \centering
    \def\arraystretch{1.4}
    \begin{tabular}{|c|c|c|c|}
        \hline
        Scenario & Device & Timer & Saved timer \\\hline\hline
        \multirow{2}{*}{Broacband}
        & Dish & T3510 & ? \\\cline{2-4}
        & AMF & T3550 & ? \\
        \hline
        \multirow{2}{*}{IoT}
        & Iridium & T3510 & ? \\\cline{2-4}
        & AMF & T3550 & ? \\
        \hline
    \end{tabular}
\end{table}

==> Tables/reg_attempts.tex <==
%! Author = arshiya
%! Date = 10/2/25
\begin{table}
	\caption{Registration Attempts}\label{tab:reg_attempts}
	\centering
	\def\arraystretch{1.6}
	\begin{tabular}{|*{7}{c|}}
		\hline
		\multirow{2}{*}{\# UEs} & \multicolumn{2}{c|}{2k} &\multicolumn{2}{c|}{3k}& \multicolumn{2}{c|}{4k}\\\cline{2-7}
		& avg & 90\%  & avg & 90\%  & avg & 90\%  \\ \hline
		\framework{}&&&&&&\\\hline
		3GPP&&&&&&\\\hline
	\end{tabular}
\end{table}
